CATS: A framework for Cooperative Autonomy Trust & Security

With cooperative perception, autonomous vehicles can wirelessly share sensor data and representations to overcome sensor occlusions, improving situational awareness. Securing such data exchanges is crucial for connected autonomous vehicles. Existing, automated reputation-based approaches often suffer from a delay between detection and exclusion of misbehaving vehicles, while majority-based approaches have communication overheads that limits scalability. In this paper, we introduce CATS, a novel automated system that blends together the best traits of reputation-based and majority-based detection mechanisms to secure vehicle-to-everything (V2X) communications for cooperative perception, while preserving the privacy of cooperating vehicles. Our evaluation with city-scale simulations on realistic traffic data shows CATS's effectiveness in rapidly identifying and isolating misbehaving vehicles, with a low false negative rate and overheads, proving its suitability for real world deployments.

==> sections/evals/certsizes.tex <==
\parab{Certificate sizes. }
We also performed size analysis of \sysname certificates that carries the signed trust attribute, and one UUID attribute that is used as an identifier of the certificate. Table \ref{tab:certsizes} summarizes our findings, showing that reasonably secure EC certificates are small enough to be transmitted in one packet, making beaconing of certificates possible.

\begin{table}
  \centering
  \begin{tabular}{@{}lll@{}}
      \toprule
      Algorithm       & \begin{tabular}[c]{@{}l@{}}Security strength (bits)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Certificate size (bytes)\end{tabular} \\ \midrule
      secp224r1       & 112                       & 501                       \\
      brainpoolP256r1 & 128                       & 530                       \\
      secp384r1       & 192                       & 611                       \\
      brainpoolP512r1 & 256                       & 709                       \\ \bottomrule
    \end{tabular}
  \vspace{1mm}
  \caption{\sysname certificate sizes with different algorithms.}
  \label{tab:certsizes}
\end{table}
% \vspace{-4mm}

==> sections/evals/crypto.tex <==
\subsection{Cryptography evaluation}
\label{sec:certeval}

\parab{Data verification time. }
We validated \sysname's certificate, signature, and trust state verification time by implementing these functions as a standalone single-threaded test application, and testing them on 3 systems with different processors that are likely representative of different classes of processors that may be found in different levels~\cite{J3016} of autonomous vehicles:

\begin{itemize}[leftmargin=*]
    \item Intel Core i7-11800H (2.3 GHz; laptop), representative of lower-end vehicle class, e.g., those at SAE level 3.
    \item AMD Threadripper 3970X (3.7 GHz; desktop), representative of server-class processors reportedly deployed in SAE level 4 autonomous vehicles \cite{WaymoXeon}.
    \item AMD Ryzen 9 7900X (4.7 GHz; desktop), representative of future SAE level 4 or 5 autonomous vehicles that will run processors with higher base clocks.
\end{itemize}

Figure \ref{fig:cert-validation-time} summarizes our findings. We observed that none of the 3 processors tested exceeds 10 milliseconds of verification time, regardless of the underlying certificate algorithm, which allows \sysname to be integrated into autonomous driving stacks without significantly increasing end-to-end latency. 

\begin{figure}[t]
    \centering
    \includegraphics[width=7.5cm]{figures/certValidationTime/cert_validation_time.png}
    \caption{\sysname validation time evaluation.}
    \label{fig:cert-validation-time}
\end{figure}

==> tables/comparison-tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

\begin{table*}
\centering
\begin{tabular}{ll|llll|llll}
\hline
                                &                                & \multicolumn{4}{c|}{\textbf{Berlin}}                                                                                                                                                          & \multicolumn{4}{c}{\textbf{Boston}}                                                                                                                                                           \\ \cline{3-10} 
                                &                                & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{\VR} & \multicolumn{1}{l|}{\VR} &                                & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{\VR} & \multicolumn{1}{l|}{\VR} &                                \\
\multirow{-3}{*}{\% Bad Sensor} & \multirow{-3}{*}{\% Flip-Flop} & \multicolumn{1}{l|}{\multirow{-2}{*}{\sysname}} & \multicolumn{1}{l|}{$\psi_{nf} = 2$}          & \multicolumn{1}{l|}{$\psi_{nf} = 100$}                                & \multirow{-2}{*}{TruPercept}   & \multicolumn{1}{l|}{\multirow{-2}{*}{\sysname}} & \multicolumn{1}{l|}{$\psi_{nf} = 2$}          & \multicolumn{1}{l|}{$\psi_{nf} = 100$}                                & \multirow{-2}{*}{TruPercept}   \\ \hline
0.1                             & 0.1                            & {\color[HTML]{036400} 0.0001}               & {\color[HTML]{CB0000} 1.4018}         & {\color[HTML]{CB0000} 15.0692}                                & {\color[HTML]{CB0000} 9.5228}  & {\color[HTML]{036400} 0.0071}               & {\color[HTML]{CB0000} 7.6814}         & {\color[HTML]{CB0000} 20.1329}                                & {\color[HTML]{CB0000} 16.7042} \\
1                               & 1                              & {\color[HTML]{036400} 0.0055}               & {\color[HTML]{CB0000} 1.5737}         & {\color[HTML]{CB0000} 19.9571}                                & {\color[HTML]{CB0000} 10.5927} & {\color[HTML]{036400} 0.0157}               & {\color[HTML]{CB0000} 6.6685}         & {\color[HTML]{CB0000} 20.7971}                                & {\color[HTML]{CB0000} 18.2571} \\
2.5                             & 2.5                            & {\color[HTML]{036400} 0.0051}               & {\color[HTML]{CB0000} 1.3136}         & {\color[HTML]{CB0000} 19.3887}                                & {\color[HTML]{CB0000} 10.4319} & {\color[HTML]{036400} 0.0271}               & {\color[HTML]{CB0000} 7.0842}         & {\color[HTML]{CB0000} 21.33}                                  & {\color[HTML]{CB0000} 18.5957} \\
1                               & 4                              & {\color[HTML]{036400} 0.0069}               & {\color[HTML]{CB0000} 1.8555}         & {\color[HTML]{CB0000} 24.1356}                                & {\color[HTML]{CB0000} 15.607}  & {\color[HTML]{036400} 0.0283}               & {\color[HTML]{CB0000} 8.7333}         & {\color[HTML]{CB0000} 27.7517}                                & {\color[HTML]{CB0000} 27.3016} \\
4                               & 1                              & {\color[HTML]{036400} 0.0038}               & {\color[HTML]{CB0000} 0.9102}         & {\color[HTML]{CB0000} 15.3072}                                & {\color[HTML]{CB0000} 6.0759}  & {\color[HTML]{036400} 0.0171}               & {\color[HTML]{CB0000} 5.9385}         & {\color[HTML]{CB0000} 18.85}                                  & {\color[HTML]{CB0000} 12.5642} \\
10                              & 10                             & {\color[HTML]{036400} 0.0073}               & {\color[HTML]{CB0000} 0.7445}         & {\color[HTML]{CB0000} 17.9461}                                & {\color[HTML]{CB0000} 9.6672}  & {\color[HTML]{036400} 0.142}                & {\color[HTML]{CB0000} 5.85}           & {\color[HTML]{CB0000} 19.864}                                 & {\color[HTML]{CB0000} 17.664}  \\ \hline
\end{tabular}
\caption{Average false negative percentages (bad messages not filtered) - lower is better, lowest value highlighted.}
\label{tab:false-negative-ratio}
\end{table*}

\usepackage[table,xcdraw]{xcolor}
\begin{table*}
\centering
\begin{tabular}{ll|llll|llll}
\hline
                                &                                & \multicolumn{4}{c|}{\textbf{Berlin}}                                                                                                                                                          & \multicolumn{4}{c}{\textbf{Boston}}                                                                                                                                                           \\ \cline{3-10} 
                                &                                & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{\VR} & \multicolumn{1}{l|}{\VR} &                                & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{\VR} & \multicolumn{1}{l|}{\VR} &                                \\
\multirow{-3}{*}{\% Bad Sensor} & \multirow{-3}{*}{\% Flip-Flop} & \multicolumn{1}{l|}{\multirow{-2}{*}{\sysname}} & \multicolumn{1}{l|}{$\psi_{nf} = 2$}          & \multicolumn{1}{l|}{$\psi_{nf} = 100$}                                & \multirow{-2}{*}{TruPercept}   & \multicolumn{1}{l|}{\multirow{-2}{*}{\sysname}} & \multicolumn{1}{l|}{$\psi_{nf} = 2$}          & \multicolumn{1}{l|}{$\psi_{nf} = 100$}                                & \multirow{-2}{*}{TruPercept}   \\ \hline
0.1                             & 0.1                            & {\color[HTML]{036400} 0.0333}                   & {\color[HTML]{CB0000} 0.8745}        & {\color[HTML]{036400} 0.0103}                    & {\color[HTML]{CB0000} 7.3023} & {\color[HTML]{036400} 0.0471}                   & {\color[HTML]{CB0000} 0.3171}                   & {\color[HTML]{036400} 0.0086}                                           & {\color[HTML]{CB0000} 0.7857} \\
1                               & 1                              & {\color[HTML]{036400} 0.2888}                   & {\color[HTML]{CB0000} 10.0417}       & {\color[HTML]{036400} 0.0840}                    & {\color[HTML]{CB0000} 7.5060} & {\color[HTML]{036400} 0.4214}                   & {\color[HTML]{CB0000} 4.7757}                   & {\color[HTML]{036400} 0.1400}                                           & {\color[HTML]{CB0000} 0.8586} \\
2.5                             & 2.5                            & {\color[HTML]{036400} 0.7215}                   & {\color[HTML]{CB0000} 23.9163}       & {\color[HTML]{036400} 0.2419}                    & {\color[HTML]{CB0000} 7.8409} & {\color[HTML]{036400} 0.9885}                   & {\color[HTML]{CB0000} 13.0057}                  & {\color[HTML]{036400} 0.3357}                                           & {\color[HTML]{CB0000} 0.9728} \\
1                               & 4                              & {\color[HTML]{036400} 0.4632}                   & {\color[HTML]{CB0000} 11.4657}       & {\color[HTML]{036400} 0.3538}                    & {\color[HTML]{CB0000} 7.6608} & {\color[HTML]{036400} 0.6483}                   & {\color[HTML]{CB0000} 4.4550}                   & {\color[HTML]{036400} 0.4416}                                           & {\color[HTML]{CB0000} 1.0383} \\
4                               & 1                              & {\color[HTML]{036400} 1.0462}                   & {\color[HTML]{CB0000} 36.2922}       & {\color[HTML]{036400} 0.0891}                    & {\color[HTML]{CB0000} 8.0458} & {\color[HTML]{036400} 1.2657}                   & {\color[HTML]{CB0000} 19.8857}                  & {\color[HTML]{036400} 0.1971}                                           & {\color[HTML]{CB0000} 0.9000} \\
10                              & 10                             & {\color[HTML]{036400} 2.8953}                   & {\color[HTML]{CB0000} 52.4282}       & {\color[HTML]{036400} 0.9689}                    & {\color[HTML]{CB0000} 9.6289} & {\color[HTML]{036400} 3.8700}                   & {\color[HTML]{CB0000} 38.9400}                  & {\color[HTML]{036400} 1.4880}                                           & {\color[HTML]{CB0000} 1.6200} \\ \hline
\end{tabular}
\caption{Average false positive percentages (good messages dropped) - lower is better, lowest value highlighted.}
\label{tab:false-positive-ratio}
\end{table*}

==> tables/time-to-ban.tex <==
\begin{table}[!htp]
  \resizebox{0.95\columnwidth}{!}{%
    \begin{tabular}{@{}ll|ll|ll|ll@{}}
      \toprule
      \multirow{2}{*}{\shortstack{\% Bad\\sensor}} & \multirow{2}{*}{\shortstack{\% Flip-\\flop}} & \multicolumn{2}{l|}{Average (seconds)} & \multicolumn{2}{l|}{Maximum (seconds)} & \multicolumn{2}{l}{$\sigma$} \\
            &       & Bad sensor & Flip-flop & Bad sensor & Flip-flop & Bad sensor & Flip-flop \\ \midrule
      0.1 & 0.1 & 25.013     & 25.067    & 63         & 41        & 5.728      & 4.019     \\
      1 & 1 & 25.689     & 26.496    & 97         & 171       & 6.820      & 10.967    \\
      2.5 & 2.5 & 27.885     & 27.991    & 247        & 149       & 12.424     & 12.061    \\
      1  & 4  & 27.529     & 27.988    & 85         & 243       & 8.144      & 14.020    \\
      4  & 1  & 27.241     & 27.596    & 156        & 126       & 9.293      & 11.805    \\
      10 & 10 & 39.35      & 43.002    & 231        & 254       & 22.080     & 33.447    \\ 
      \bottomrule
    \end{tabular}
  }
  \vspace{1mm}
  \caption{Time taken for \sysname to ban vehicles - Berlin scenario.}
  \label{tab:time-to-ban}
\end{table}

\begin{table}[!htp]
  \resizebox{0.95\columnwidth}{!}{%
    \begin{tabular}{@{}ll|ll|ll|ll@{}}
      \toprule
      \multirow{2}{*}{\shortstack{\% Bad\\sensor}} & \multirow{2}{*}{\shortstack{\% Flip-\\flop}} & \multicolumn{2}{l|}{Average (seconds)} & \multicolumn{2}{l|}{Maximum (seconds)} & \multicolumn{2}{l}{$\sigma$} \\
            &     & Bad sensor & Flip-flop & Bad sensor & Flip-flop & Bad sensor & Flip-flop \\ \midrule
        %           -----   avg   -----     -----   max   -----       -----   stdev   -----
        0.1 & 0.1 & 38.462     & 49.158    & 350        & 644       & 38.974     & 76.027    \\
        1 & 1     & 42.777     & 43.120    & 407        & 364       & 34.658     & 38.503    \\
        2.5 & 2.5 & 44.299     & 48.063    & 363        & 485       & 35.483     & 48.067    \\
        1  & 4    & 42.937     & 48.106    & 258        & 486       & 31.572     & 46.675    \\
        4  & 1    & 43.861     & 45.362    & 507        & 293       & 37.785     & 39.452    \\
        10 & 10   & 54.205     & 57.649    & 518        & 541       & 44.808     & 54.768    \\ \bottomrule
    \end{tabular}
  }
  \vspace{1mm}
  \caption{Time taken for \sysname to ban vehicles - Boston scenario.}
  \label{tab:time-to-ban-boston}
\end{table}
